Training-Free Action Recognition and Goal Inference with Dynamic Frame Selection

We introduce VidTFS, a Training-free, open-vocabulary video goal and action inference framework that combines the frozen vision foundational model (VFM) and large language model (LLM) with a novel dynamic Frame Selection module. Our experiments demonstrate that the proposed frame selection module improves the performance of the framework significantly. We validate the performance of the proposed VidTFS on four widely used video datasets, including CrossTask, COIN, UCF101, and ActivityNet, covering goal inference and action recognition tasks under open-vocabulary settings without requiring any training or fine-tuning. The results show that VidTFS outperforms pretrained and instruction-tuned multimodal language models that directly stack LLM and VFM for downstream video inference tasks. Our VidTFS with its adaptability shows the future potential for generalizing to new training-free video inference tasks.

==> tables/ablation_alignment_between_visual.tex <==
\begin{table}[tb]

\centering
\resizebox{\textwidth}{!}{\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule 
 \multirow{2}{*}{\textbf{Method}} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 0.1} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 0.3} & 
 \multicolumn{5}{c}{\begin{math}\rho\end{math} = 0.5} \\
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}   
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}} 
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}\\
 \midrule
w/o ES & & & & & &
 & & & & & 
 & & & & \\
ES (Caption Steps) & & & & & & 
 & & & & & 
 & & & & \\
\textbf{ES (VisualxSteps)} & & & & & & & & & & & 
 & & & & \\
 \bottomrule
\end{tabular}}
\centering

\caption{Ablation study of the evidence selector (ES) component. We report following metrics: SPICE (S), CIDEr (C), METEOR (M), BERTScore (B), and SBERT (SB).} 
\label{tab:ablation_evidence_selector}
\end{table}

==> tables/ablation_evidence_selector_additional.tex <==
\begin{table}[t]


\centering
\scriptsize


\vspace{5pt}
\resizebox{\textwidth}{!}{
\begin{subtable}
\centering
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule 
 \multirow{2}{*}{\textbf{COIN}} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 10\%} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 30\%} & 
 \multicolumn{5}{c}{\begin{math}\rho\end{math} = 50\%} \\
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}   
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}} 
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}\\
 \midrule
w/o ES & 18.3 & 52.8 & 11.4 & 23.0 & 41.9 
& 21.0 & 63.2 & 12.7 & 26.7 & 46.1
& 22.0 & 68.2 & 13.2 & 27.8 & 47.7
\\

\textbf{with ES}& \textbf{20.4} & \textbf{62.6} & \textbf{12.5} & \textbf{27.2} & \textbf{45.0}
& \textbf{23.0} & \textbf{71.4} & \textbf{13.7} & \textbf{30.4} & \textbf{49.6}
& \textbf{25.1} & \textbf{76.7} & \textbf{14.3} & \textbf{31.6} & \textbf{51.5}
\\

 \bottomrule
\end{tabular}

\end{subtable}
}

(a) Goal inference on COIN dataset


\vspace{5pt}
\begin{subtable}
\centering
\begin{tabular}{l|ccccc}
\toprule 
 \multirow{2}{*}{\textbf{ActivityNet}} & 
 \multicolumn{5}{c}{\begin{math}\rho\end{math} = 100\%} \\

 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}\\
 \midrule
w/o ES & 21.2 & 79.6 & 12.7 & 22.3 & 57.4 \\

\textbf{with ES}& \textbf{24.0} & \textbf{94.0} & \textbf{14.7} & \textbf{28.8} & \textbf{61.0} \\
 \bottomrule

\end{tabular}
\end{subtable}%

(b) Action recognition on Activitynet dataset
    
\centering

\caption{Ablation study of the evidence selector (ES) component on COIN and ActivityNet.}
\label{tab:ablation_evidence_selector_additional}
\end{table}

==> tables/ablation_inter_output.tex <==
%\begin{table}[t]
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{cccc|cccc|cccc}
\toprule 
 \multicolumn{4}{c|}{\begin{math}\rho\end{math} = 10\%} & 
 \multicolumn{4}{c|}{\begin{math}\rho\end{math} = 30\%} & 
 \multicolumn{4}{c}{\begin{math}\rho\end{math} = 50\%} \\
 
 {$\mathcal{H}$} & {$\mathcal{\ddot{H}}$} & {$h_c$} & {$h$}  &
 {$\mathcal{H}$} & {$\mathcal{\ddot{H}}$} & {$h_c$} & {$h$}  &
 {$\mathcal{H}$} & {$\mathcal{\ddot{H}}$} & {$h_c$} & {$h$}   \\

 \midrule
 &  &  & & 
 &  &  & & 
 &  &  & \\
\bottomrule
\end{tabular}
%\end{table}

\caption{Analysis on intermediate inference output. We report the SBERT score.}
\label{tab:ablation_inter}
\end{table}



==> tables/ablation_remove_repeat_captions.tex <==
\begin{table}[t]
\centering
\scriptsize{
\resizebox{\textwidth}{!}{\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule 
 \multirow{2}{*}{\textbf{Method}} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 10\%} & 
 \multicolumn{5}{c|}{\begin{math}\rho\end{math} = 30\%} & 
 \multicolumn{5}{c}{\begin{math}\rho\end{math} = 50\%} \\
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}   
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}} 
 
 & \multirow{1}{*}{\footnotesize{S}} & \multirow{1}{*}{\footnotesize{C}} 
 & \multirow{1}{*}{\footnotesize{M}} & \multirow{1}{*}{\footnotesize{B}} & \multirow{1}{*}{\footnotesize{SB}}\\

 \midrule

Remain repeat caption & 21.1 & 69.2 & 14.8 & 29.5 & 45.6
& 19.2 & 73.3 & 14.7 & 29.7 & 46.6
& 21.1 & 76.2 & 15.8 & 32.1 & 48.8
\\

Removed repeat caption & \textbf{23.0} & \textbf{80.1} & 15.4 & \textbf{32.3} & \textbf{47.6} 
& \textbf{23.1} & \textbf{91.7} & \textbf{16.9} & \textbf{35.0} &
\textbf{50.9} & \textbf{24.4} & \textbf{80.8} & \textbf{16.3} & \textbf{34.5} &
\textbf{50.2}
\\

 \bottomrule
\end{tabular}}
}

\centering
\caption{Ablation on repeated captions.}
\label{tab:ablation_remove_repeat_caption}
\end{table}

==> tables/accuracy_by_SBERT_match.tex <==
%\begin{table}[t]
\begin{table}[h]


\scriptsize
\centering
\begin{tabular}{l|ccc|ccc|c|c}
  \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{\textbf{CrossTask}}& \multicolumn{3}{c|}{\textbf{COIN}} & \textbf{UCF101} & \textbf{ActivityNet}\\
    
    
    & \multirow{1}{*}{10\%} 
    & \multirow{1}{*}{30\%} 
    & \multirow{1}{*}{50\%} 
    & \multirow{1}{*}{10\%} 
    & \multirow{1}{*}{30\%} 
    & \multirow{1}{*}{50\%}
    & \multirow{1}{*}{100\%}
    & \multirow{1}{*}{100\%}\\
    
    \midrule
    BLIP-2\cite{li2023blip}& 35.9 & 37.0 & 37.7 & 36.7 & 36.3 & 37.3 & 56.5 & 43.5 \\
    InstructBLIP\cite{instructBLIP}& 36.0 & 32.5 & 33.3 & 34.8 & 33.1 & 33.8 & 42.5 & 25.2\\
    Video-ChatGPT\cite{videochatgpt}& 38.0 & 36.8 & 36.0 & 39.6 & 39.7 & 39.1 & 54.2 & 33.9\\
    mPLUG-Owl \cite{Ye2023mPLUGOwlME}& 50.1 & 53.5 & 49.9 & 41.5 & 48.8 & 51.1 & \textbf{56.9} & 48.1\\
    Video-LLaVA \cite{lin2023video}& 44.5 & 44.2 & 45.3 & 51.6 & \textbf{51.9} & 50.8 & 53.4 & \textbf{56.8}\\
    mPLUG-Owl+V13B & \textbf{52.4} & \textbf{56.4} & \textbf{51.6} & \textbf{51.6} & 50.6 & 52.3 & 41.2 & 40.3\\
    \midrule
    VidTFS (V13B) & 51.8 & 53.5 & 49.9 & 46.3 & 50.3 & \textbf{52.8} & 44.0 & 37.2\\
    \bottomrule
  \end{tabular}

\caption{Evaluation.}
\label{tab:accuracy_by_sbert_match}
\end{table}




==> tables/llm_prompt_llama3_eval_acc.tex <==
\begin{table}[tb!]


% \scriptsize



    Prompt  \\
    

    I want to perform <TASK NAME> after observing some visual descriptions.

    <ICL EXAMPLE>
    
    Based on the description: < $\mathcal{D}$ or $\ddot{\mathcal{D}}$ >
    
    \{Based on these options: <$\mathcal{H}$ / $\mathcal{\ddot{H}}$>\}
    
    List the most likely <K NUMBER> correct <TARGET> without any explanation. Answer: \\
    
    


  
\caption{ICL}
\label{tab:llm_icl}
\end{table}

==> tables/zseap_ar_c_table.tex <==
\begin{table}
\centering
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Method & UCF101 & ActivityNet\\
    \midrule
    ViFi-CLIP & 67.6 & 51.7\\
    XCLIP & 63.5 & 46.2\\
    MAXI & 69.8 & 52.4\\
    \midrule
    ZERO (V13B) & & \\
    \bottomrule
  \end{tabular}
\label{tab:close_ended_actions_ucf101}
\caption{Close-ended zero-shot action recognition results on UCF101 and ActivityNet dataset. We report top@1 accuracy.}
\label{tab:close_ended_action_recognition}
\end{table}

==> tables/zsgoalc_table.tex <==
%\begin{table}[t]
\begin{table}


\scriptsize
\centering
\begin{tabular}{l|ccc|ccc}
  \toprule
    \multirow{3}{*}{Method} & \multicolumn{3}{c|}{\textbf{CrossTask}}& \multicolumn{3}{c}{\textbf{COIN}}\\
    & \multicolumn{3}{c|}{Observation ratio} 
    & \multicolumn{3}{c}{Observation ratio}\\
    
    & \multirow{1}{*}{10\%} 
    & \multirow{1}{*}{30\%} 
    & \multirow{1}{*}{50\%} 
    & \multirow{1}{*}{10\%} 
    & \multirow{1}{*}{30\%} 
    & \multirow{1}{*}{50\%}\\
    
    \midrule
    ViFi-CLIP \cite{vificlip}& & & & & &\\
    X-CLIP \cite{xclip}& & & & & &\\
    MAXI \cite{MAXI}& & & & & &\\
    \midrule
    VidTFS (V13B) & & & & & &\\
    \textbf{VidTFS (GPT-3.5)} & & & & & &\\
    \bottomrule
  \end{tabular}

\caption{Accuracy results of close-ended goal inferences on CrossTask and COIN dataset.}
\label{tab:close_ended_goal_inference}
\end{table}
